Generating Symbolic World Models via Test-time Scaling of Large Language Models

Solving complex planning problems requires Large Language Models (LLMs) to explicitly model the state transition to avoid rule violations, comply with constraints, and ensure optimality-a task hindered by the inherent ambiguity of natural language. To overcome such ambiguity, Planning Domain Definition Language (PDDL) is leveraged as a planning abstraction that enables precise and formal state descriptions. With PDDL, we can generate a symbolic world model where classic searching algorithms, such as A*, can be seamlessly applied to find optimal plans. However, directly generating PDDL domains with current LLMs remains an open challenge due to the lack of PDDL training data. To address this challenge, we propose to scale up the test-time computation of LLMs to enhance their PDDL reasoning capabilities, thereby enabling the generation of high-quality PDDL domains. Specifically, we introduce a simple yet effective algorithm, which first employs a Best-of-N sampling approach to improve the quality of the initial solution and then refines the solution in a fine-grained manner with verbalized machine learning. Our method outperforms o1-mini by a considerable margin in the generation of PDDL domains, achieving over 50\% success rate on two tasks (i.e., generating PDDL domains from natural language description or PDDL problems). This is done without requiring additional training. By taking advantage of PDDL as state abstraction, our method is able to outperform current state-of-the-art methods on almost all competition-level planning tasks.

==> content/exp.tex <==
% \section{Experiments on Domain Generation}
% In this section, we answer how effectively our method synthesizes competition-level PDDL domains.
% We present two testing tasks for PDDL generation: 1. NL2Domain: translating natural language to PDDL domains and 2. Prob2Domain: generating PDDL domains from PDDL problems. 

% \subsection{Benchmarks}
% \label{benchmarks}
% NL2Domain assesses the LLMs' ability to autoformalize the PDDL planning domain based on natural language description. 
% Prob2Domain assesses the LLMs' ability to infer the underlying domain definitions solely from given PDDL problem files. 
% We adopt international planning competitions test cases\footnote{https://github.com/potassco/pddl-instances} as the test dataset, which comprises 332 PDDL problem codes and 283 ground truth PDDL domain codes. 
% To obtain a natural language description, we utilize GPT-4o~\cite{achiam2023gpt} the informalizer to translate the PDDL domain back into natural language.

% \subsection{Baselines}
% The baselines involve general LLMs, specifically, Qwen2.5 families~\cite{yang2024qwen2}, Llama3.1families~\cite{dubey2024llama}, Yi families~\cite{young2024yi}, and GPT-4o~\cite{achiam2023gpt}.
% We also include code LLM such as Qwen2.5-Coder, and Yi-1.5-Coder.
% Significantly, we also compare with large reasoning language models (LRM) o1.

% \subsection{Metrics}
% VAL~\cite{howey2003val} is adopted as a syntax checker for the generated PDDL domains. 
% It verifies that all required components, such as predicates, actions, and initial states, are correctly defined according to PDDL syntax rules. 
% We set the pass rate of VAL for each LLM as a metric to evaluate the performance of LLMs on PDDL domain synthesis. 


% \subsection{Numerical Results}
% \label{result}
% As shown in Table~\ref{tab:main-results}.
% Among the open-source models evaluated, most exhibit limited effectiveness, with numerous configurations recording scores of 0.0 across both NL2Domain and Problem2Domain benchmarks. 
% Notably, larger parameter models such as the 72B Qwen2.5-Instruct only gets 38.5 on NL2Domain, and 32.8 on Prob2Domain.
% On the other hand, Coder models demonstrate enhanced capabilities compared to similar scale instruct models, achieving higher scores by effectively leveraging their pretrained knowledge tailored for coding tasks.
% Our proposed methods significantly outperform both open-source and closed-source models.
% The System 2 approach we adopted, which integrates BoN sampling and VGD, consistently yields superior results across various parameter scales.
% For instance, the BoN-8-Qwen2.5-Instruct model with 7B parameters attains a score of 9.2 on NL2Domain and 34.6 on Problem2Domain, which substantially surpasses the baseline models. 
% Scaling up to 14B and 72B parameters, our methods achieve remarkable scores of 51.6 and 56.2 on NL2Domain, and 62.0 and 71.1 on Problem2Domain, respectively. 
% Moreover, the VGD-enhanced models exhibit even greater performance improvements, with the VGD-5-BoN-8-Qwen2.5-Coder model reaching scores of 85.2 on NL2Domain and 71.4 on Problem2Domain.
% \begin{table}[ht]
% \centering
% \caption{\small Comparison of the performance on PDDL Domain synthesis.}
% \label{tab:main-results}
% \begin{tabular}{lcccc}
% \hline
% Model                     & \# Params & NL2Domain                                      & Problem2Domain          & Avg.                 \\ \hline
%                           &           & \multicolumn{1}{l}{\textit{Open-Source Models}} & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{} \\ \hline
% Qwen2.5-Instruct          & 0.5B      & 0.0                                            & 0.0                     & 0.0                  \\
% Qwen2.5-Instruct          & 1.5B      & 0.0                                            & 0.0                     & 0.0                  \\
% Qwen2.5-Instruct          & 3B        & 2.1                                            & 1.5                     & 0.0                  \\
% Qwen2.5-Instruct          & 7B        & 5.7                                            & 11.7                     & 8.7                  \\
% Qwen2.5-Instruct          & 14B       & 21.6                                           & 25.3                    & 23.5                 \\
% Qwen2.5-Instruct          & 32B       & 24.0                                           & 31.6                    & 27.8                 \\
% Qwen2.5-Instruct          & 72B       & 38.5                                           & 32.8                    & 35.7                 \\
% Qwen2.5-Coder             & 1.5B      & 0.0                                            & 0.0                     & 0.0                  \\
% Qwen2.5-Coder             & 7B        & 21.9                                           & 18.4                    & 20.2                 \\ \hline
% Llama3.1-Instruct         & 8B        & 0.0                                            & 0.0                     & 0.0                  \\
% Llama3.1-Instruct         & 70B       & 1.1                                            & 0.0                     & 0.6                  \\ \hline
% Yi-1.5-Chat               & 6B        & 0.4                                            & 1.8                     & 1.1                  \\
% Yi-1.5-Chat               & 9B        & 6.7                                            & 9.3                     & 8.0                  \\
% Yi-1.5-Chat               & 34B       & 12.0                                           & 8.7                     & 10.4                  \\
% Yi-Coder                  & 1.5B      & 0.0                                            & 0.0                     & 0.0                  \\
% Yi-Coder                  & 9B        & 9.9                                            & 14.5                    & 12.2                  \\ \hline
% \textbf{}                 &           & \multicolumn{1}{l}{\textit{Closed-Source Models}}        & \multicolumn{1}{l}{}    &                      \\ \hline
% GPT-4o                    & -         & 5.3                                            & 50.0 & 27.7                  \\
% o1-mini                   & -         & 41.7                                           & 33.7 & 37.7                  \\ 
% o1-preview          & -    & 55.8 & 52.4 & 54.1 \\ 
% \hline
%                           &           & \multicolumn{1}{l}{\textit{Our Methods}}       & \multicolumn{1}{l}{}    &                      \\ \hline
% % BoN-8-Qwen2.5-Instrcut    & 7B       & 2.5（+1.4）  & 15.7 (+11.6)  & 9.1 (+6.5)  \\
% BoN-8-Qwen2.5-Instrcut    & 0.5B      & 0.0 (+0.0)                                    & 0.0 (+0.0)            & 0.0    \\
% BoN-8-Qwen2.5-Instrcut    & 1.5B      & 2.1 (+2.1)                                    & 0.3 (+0.3)            & 1.2             \\
% BoN-8-Qwen2.5-Instrcut    & 3B        & 11.7 (+9.5)                                   & 1.2 (+0.3)            & 6.5       \\
% BoN-8-Qwen2.5-Instrcut    & 7B        & 9.2 (+3.5)                                     & 34.6 (+22.9)            & 21.9       \\
% BoN-8-Qwen2.5-Instrcut    & 14B       & 51.6 (+30.0)                                   & 62.0 (+36.7)            &   56.8           \\
% BoN-8-Qwen2.5-Instrcut    & 32B       & 66.8 (+46.7)                                   & 71.1 (+39.5)            & 70.9       \\
% BoN-8-Qwen2.5-Instruct    & 72B       & 60.8 (+22.3)                                   & 73.8 (+41.0)            & 67.3      \\
% BoN-8-Qwen2.5-Coder       & 7B        & 73.1 (+51.2)                                   & 63.3 (+44.9)            & 68.2       \\
% VGD-5-BoN-8-Qwen2.5-Instruct & 0.5B        & 0.0 (+0.0)                                & 0.0 (+0.0)     & 0.0        \\ 
% VGD-5-BoN-8-Qwen2.5-Instruct & 1.5B        & 2.8 (+2.8)                               & 0.3 (+0.3)     & 1.6         \\ 
% VGD-5-BoN-8-Qwen2.5-Instruct & 3B        & 18.7 (+16.6)                               & 1.8 (+0.3)     & 10.3         \\
% VGD-5-BoN-8-Qwen2.5-Instruct & 7B        & 21.9 (+16.2)                                & 49.1 (+37.3)     & 35.5      \\ 
% VGD-5-BoN-8-Qwen2.5-Instruct & 14B        & 77.0 (+55.4)                               & 80.4 (+55.1)     &   78.7      \\ 
% VGD-5-BoN-8-Qwen2.5-Instruct & 32B        & 86.2 (+62.2)                               & 90.9 (+59.3)     & 88.6         \\ 
% VGD-5-BoN-8-Qwen2.5-Instruct & 72B        & 78.4 (+39.9)                              & 86.4  (+53.6)     & 82.4        \\ 
% VGD-5-BoN-8-Qwen2.5-Coder & 7B        & 85.2 (+63.3)                                   & 71.4 (+53.0)            & 78.3         \\ \hline

% \end{tabular}
% \end{table}

% \section{Ablation Study: Test Time Computation Scaling}
% ~\label{model_setup}
% In this section, we delve into an ablation study focusing on the test-time computation scaling of our synthesis framework. The computational resources are primarily influenced by two key factors:
% $N$: This represents the number of searches conducted via Best-of-N sampling.
% $E$: This indicates the number of epochs utilized in VGD for refining thoughts and domains.
% The objective of this study is to analyze how variations in both variables affect the performance of synthesizing PDDL. 
% By systematically adjusting these parameters, we aim to ascertain their impact on downstream results.

% We leverage the Qwen2.5-7B-Coder as the base model. 
% The hyperparameters when sampling are: 
% 1. temperature: we set the temperature parameter to 0.7 to retain randomness in the generated output. 
% 2. top-p (Nucleus Sampling): we utilize top-p sampling with a parameter of 0.9 to ensure that we consider the most likely tokens based on their cumulative probability.
% 3. maximum token length: the maximum token length is set to 2,048 tokens to generate long outputs.

% \textbf{Ablate Sampling Numbers.} In the first experiment, we explore how the performance of BoN varies with increasing $ N $.
% Figure~\ref{ablate} presents the number of samples that pass the VAL checking as the sample size increases. 
% We observe that performance generally improves as $ N $ increases from 1 to 32. 
% However, as $ N $ continues to grow beyond this point, reaching up to 256, the performance levels off and even slightly declines. 
% This suggests that there is an optimal range for $ N $ where the performance benefits are maximized without incurring unnecessary computational overhead. 
% Notably, even with BoN alone, the Qwen2.5-7B-Coder model is capable of successfully generating 95.8\% and 89.2\% of PDDL domains for NL2Domain and Prob2Domain, respectively.
% % \begin{wrapfigure}{r}{0.5\textwidth}
% %     \centering
% %     \includegraphics[width=0.6\linewidth]{content/imgs/qwenscale.png}
% %     \caption{The trend of increasing sampling numbers}
% %     \label{fig:bon}
% % \end{wrapfigure}

% \textbf{Ablate VGD Epochs.} We investigate how the performance of VGD varies with the number of update epochs $E$. 
% We employ VGD, in which the critique LLMs are the same models as the generator LLMs, and we keep the same decoding hyperparameters as the generator LLMs (see Section~\ref{model_setup}).
% We obtain the results after applying BoN-8-Qwen2.5-Coder and adopt VGD to improve the domain generations further, as shown in Figure~\ref{ablate}.
% % \begin{wrapfigure}{r}{0.5\textwidth}
% %     \centering
% %     \includegraphics[width=0.6\linewidth]{content/imgs/GD_Samp.png}
% %     \caption{Performance trend with increasing update epochs}
% %     \label{fig:vgd}
% % \end{wrapfigure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.9\linewidth]{content/imgs/GD_Samp.pdf}
%     \caption{\small Left: Performance trend with increasing update epochs. Right: The trend of increasing sampling numbers.}
%     \label{ablate}
% \end{figure}
% The baseline represents the number of accurate domains after BoN.
% As the number of epochs increases, both NL2Domain and Prob2Domain show an upward trend, suggesting that the self-improvement process is effective in enhancing the performance of domain generation, although the rate of increase remains relatively steady.
% Finally, the percentage of accurate domains converges at 97.5\% for NL2Domain and 92.7\% for Prob2Domain.
% BoN shows earlier saturations than VGD.
% The insight here is that BoN is a good enough algorithm for PDDL generation, and VGD can be used as a further improvement tool to increase performance.


% \section{Ablation Study: Model Parameters Scaling}
% \subsection{Experiment Setup}
% In this section, we conduct experiments to analyze the impact of the base model size on the quality of generated PDDL domains when using BoN sampling and VGD for self-improvement. 
% And compare the model parameter scaling with test time computation scaling.
% We utilize base models from the Qwen2.5-Instruct series.
% We leverage the same dataset as described in Section~\ref{benchmarks}.
% % \begin{wrapfigure}{r}{0.6\textwidth}
% %     \centering
% %     \includegraphics[width=0.9\linewidth]{content/imgs/Qwen2.5-Instruct.png}
% %     \caption{BoN Performance trend with increasing model parameters.}
% %     \label{fig:param}
% % \end{wrapfigure}

% \subsection{Numerical Results}
% \textbf{BoN Sampling.}
% For the BoN sampling experiments, we kept the sampling number $ N = 8 $ consistent across all base models. The results are presented in Figure~\ref{bon}. 
% Compared with the System 1 approach shown in Table~\ref{tab:main-results}, we observed that models larger than 7B exhibit significantly higher success rates. 
% Specifically, the 7B models show increases of 1.4\% and 11.6\%; the 14B models show increases of 27.2\% and 25.3\%; the 32B models achieve the most substantial improvements of 34.2\% and 39.9\%; and the 72B models show increases of 20.1\% and 34.6\%. 
% These results suggest that the performance gains from scaling model size tend to saturate around the 32B model. 
% However, the performance of models smaller than 7B remains at 0.0\% for both tasks.
% This indicates that these smaller models lack the necessary capacity to generate accurate PDDL domains, even when utilizing BoN sampling.
% Although we do not have detailed information on how the training datasets differ among the various models, we speculate the reason is smaller models have limited representational capacity compared to larger models.
% Generating syntactically correct and semantically meaningful PDDL domains requires a deep understanding of formal language structures and domain-specific knowledge, which smaller models may struggle to capture due to their reduced parameters.
% Moreover, larger models likely benefit from being trained on more extensive and diverse datasets, potentially including more examples of programming languages and formal specifications like PDDL.
% However, we found that for certain larger model sizes, scaling on test time is more optimal as Table~\ref{tab:main-results} shows that in System 1 manner, performance generally increases with larger model parameters, it is often more optimal to scale test-time computation rather than increasing model size.
% For instance, BoN-8-Qwen2.5-Instruct-14B achieves almost double the success rate compared to Qwen2.5-Instruct-72B.
% Similar patterns have been observed in prior work~\cite{snell2024scaling} on general reasoning tasks.

% \textbf{VGD.}
% % \begin{wrapfigure}{r}{0.6\textwidth}
% %     \centering
% %     \includegraphics[width=0.8\linewidth]{content/imgs/Qwen2.5-Instruct_textgard.png}
% %     \caption{VGD Peformace of Qwen Series after BoN@8.}
% %     \label{VGD}
% % \end{wrapfigure}
% \begin{figure}
%     \centering
% \includegraphics[width=0.8\linewidth]{content/imgs/Combined_BoN_VGD.pdf}
%     \caption{\small Left: BoN Performance trend with increasing model parameters. Right: VGD Peformace of Qwen Series after BoN@8.}
%     \label{bon}
% \end{figure}
% For the VGD experiments, we set the VGD number $T = 5 $ and BoN sampling number $ N = 8 $ consistent across all the Qwen2.5-instruct models.
% The results are presented in Figure~\ref{bon}. 
% The results illustrate that the VGD further improves the performance after BoN@8 for almost all the models.
% However, the performance of models smaller than 0.5B remains at 0.0\% for both tasks even when utilizing BoN sampling and VGD method. 
% This indicates that these smaller models not only lack capabilities to generate the correct PDDL domains but are also weak at self-critique the generated domains.

% \section{PDDL Problem Generations}
% Scaling test-time computation can also be effectively generalized to PDDL problem generation. 
% We adopt the benchmark from Planetarium~\cite{zuo2024planetarium}, which focuses on generating PDDL problem code from natural language descriptions. 
% The dataset is complex due to its abstractness and the longer context required for describing objects.
% The baseline methods include the Gemma 1.1 IT models with 2B and 7B parameters, and Mistral~\cite{jiang2023mistral} v0.3 Instruct 7B, both evaluated in zero-shot and fine-tuned settings. 
% Additionally, GPT-4 serves as the state-of-the-art System 1 model. 
% The results of baseline in Table~\ref{tab:model_performance} are originally from Planetarium.
% It is worth mentioning that Planetarium fine-tuned Gemma and Mistral on a training dataset of 132,027 examples of PDDL problem code, which raises concerns about overfitting, as the correct rate increases sharply from close to 0.0\% to over 94\%.
% However, as shown in Table~\ref{tab:model_performance}, despite not being fine-tuned on any PDDL problem dataset, we achieve fine-tuned-level performance by simply leveraging Best-of-N (BoN) sampling with 16 samples on Qwen2.5-Coder-7B. 
% Our method attains a correct rate of 99.24\%, surpassing even the fine-tuned models and highlighting the effectiveness of scaling test-time computation.

% \begin{table}[htbp]
% \centering
% \caption{Performance Comparison of Different Models on PDDL problem generation}
% \label{tab:model_performance}
% \begin{tabular}{l|l|c}
% \hline
% \textbf{Model} & \textbf{Setting} & \textbf{Correct Rate} \\
% \hline
% \multirow{2}{*}{Gemma 1.1 IT 2B} & Zero-shot & 0.00\% \\
%  & Fine-tuned & 94.21\% \\
% \multirow{2}{*}{Gemma 1.1 IT 7B} & Zero-shot & 0.00\% \\
%  & Fine-tuned & 98.79\% \\

% \multirow{2}{*}{Mistral v0.3 Instruct 7B} & Zero-shot & 0.01\% \\
%  & Fine-tuned & 99.00\% \\

% GPT-4o & Zero-shot & 35.12\% \\
% Ours (Qwen2.5-Coder-7B) & BoN@16 & 99.24\% \\
% \hline
% \end{tabular}
% \end{table}


==> content/problem_formulation.tex <==
% \section{Problem Formulation}

% The classical planning problem~\cite{fikes1971strips} in artificial intelligence involves finding a sequence of actions that transition an agent from an initial state to a desired goal state within a deterministic and fully observable environment. It is formalized as a tuple $\langle \mathcal{S}, \mathcal{A}, T, s_0, G \rangle$, where:
% $\mathcal{S}$ is the set of all possible states;
% $\mathcal{A}$ is the set of all possible actions;
% $T: \mathcal{S} \times \mathcal{A} \rightarrow \mathcal{S}$ is the state transition function, specifying the outcome state resulting from applying an action in a state;
% $s_0 \in \mathcal{S}$ is the initial state;
% $G$ is the goal condition, a predicate over states.
% The objective is to find a sequence of actions $a_{1}, a_{2}, \dots, a_{n} \in \mathcal{A}$ such that applying these actions successively transitions the system from $s_0$ to a state $s_n$ satisfying the goal condition $G$:
% \[
% s_n = T(s_{n-1}, a_{n}) = T(T(\dots T(T(s_0, a_1), a_2), \dots, a_{n-1}), a_{n})
% \]
% with
% \[
% s_n \models G
% \]
% Previous works that adopt LLMs as planners estimate state transitions implicitly within language latent spaces, lacking explicit representations of the state space required for classical planning. This implicit representation can make it challenging to ensure consistency, validity, and completeness in the planning process. 
% In contrast, our work leverages LLMs to generate explicit representations of the state space by creating PDDL domains. We utilize the generative capabilities of LLMs to produce formal PDDL models from high-level descriptions of the planning tasks. 
% This approach bridges the gap between natural language specifications and formal planning models.

% By generating PDDL domains using LLMs, we obtain: 1. explicit definitions of the set of states $\mathcal{S}$ through predicates and objects, 2. formal specifications of actions $\mathcal{A}$, including their preconditions and effects, 3. a deterministic state transition function $T$ derived from the action definitions, 4. abilities to cooperate with clearly defined initial state $s_0$ and goal condition $G$ in PDDL syntax.
% Thus the new objective under this background is: 
% Given high-level descriptions of planning tasks, our objective is to leverage LLMs to create PDDL domains that can represent state transitions explicitly. 
% By generating these explicit representations, we enable classical planning algorithms to efficiently search for plans using the defined state transitions during the planning process.


